Sieved Enumeration of Interval Orders and Other Fishburn Structures

Following a result of Eriksen and Sj\"{o}strand (2014) we detail a technique to construct structures following the Fishburn distribution from appropriate Mahonian structures. This technique is introduced on a bivincular pattern of Bousquet-M\'elou et al. (2010) and then used to introduce a previously unconsidered class of matchings; explicitly, zero alignment matchings according to the number of arcs which are both right-crossed and left nesting. We then define a statistic on the factorial posets of Claesson and Linusson (2011) counting the number of features which we refer to as mislabelings and demonstrate that according to the number of mislabelings that factorial posets follow the Fishburn distribution. As a consequence of our approach we find an identity for the Fishburn numbers in terms of the Mahonian numbers.

==> linear.tex <==
\newcommand{\fmt}{p_1}
\newcommand{\fmo}{p_2}
\newcommand{\mft}{q_1}
\newcommand{\mfo}{q_2}


\section*{Linear Combination of Mesh Patterns}

In order to motivate this section we briefly review the connections
between permutation patterns, Fishburn structures and the Mahonian
distribution.

Recall that contemporary study of Fishburn structures has been
motivated by the introduction of \emph{bivincular
  patterns}~\cite{two-plus-two-free}, which were in turn given as a
generalization of the \emph{vincular patterns} (n\'e
\emph{generalized patterns}) of Babson and Steingr\'imsson
\cite{babson-steingrimsson}.  Furthermore the mesh patterns of
Claesson and Br\"and\'en~\cite{meshpatterns} evolve as an abstraction
of bivincular patterns. We therefore have the following hierarchy of
patterns.

$$\mbox{classical} \subset \mbox{vincular} \subset \mbox{bivincular} \subset \mbox{mesh}$$


The introduction of vincular patterns by Babson and Steingr\'{i}msson
was in order to provide a unifying framework via permutation patterns
for certain Mahonian permutation statistics, arguably the most simple
of which is the number of inversions corresponding to the classical
pattern
\begin{center}
\pattern{}{2}{1/2,2/1}{}.
\end{center}

They identify several examples where the sum of
occurrences contained in a linear combination of vincular patterns is
used to encode both previously studied and new statistics which follow
the Mahonian distribution on permutations.

For example the \emph{major index} on permutations is defined as being
the total sum of descent positions. Babson and Steingr\'imsson
identify this as corresponding to the following linear combination of
vincular patterns,

\begin{center}
\pattern{}{3}{1/1,2/3,3/2}{2/0,2/1,2/2,2/3} +
\pattern{}{3}{1/2,2/3,3/1}{2/0,2/1,2/2,2/3} +
\pattern{}{3}{1/3,2/2,3/1}{2/0,2/1,2/2,2/3} +
\pattern{}{2}{1/2,2/1}{1/0,1/1,1/2}. 
\end{center}

As this chapter has identified an explicit link between Mahonian and
Fishburn structures and that the study of these structures has been
strongly influenced by the aforementioned hierarchy of pattern types
it is therefore natural to consider linear combinations of patterns
which follow the Fishburn distribution. This section presents one
such, non-trival example which is based upon a linear combination of
mesh patterns introduced by Claesson and
Br\"and\'en~\cite{meshpatterns}.

Claesson and Br\"and\'en demonstrate that occurrences of the following
patterns in permutations are Mahonian.

$$
\pattern{}{3}{1/2,2/3,3/1}{3/0,3/1} + \pattern{}{2}{1/2,2/1/}{2/0} 
$$

(we take a trival symmetry of the patterns appearing in the
original paper)

Checking via computer where a new entry may be inserted into the above
patterns such that the inserted entry has its value and position fixed
by pre-existing entries within the pattern leads us to conjecture the
following proposition.

\begin{proposition}\label{prop-linear-comb-mesh}
The linear combination of mesh patterns
$$
\mft + \fmo = 
\pattern {}{4}{1/3,2/4,3/2,4/1}
           {2/0,2/1,2/2,2/3,2/4,0/2,1/2,3/2,4/2,4/0,4/1}
  +  
  \pattern{}{3}{1/2,2/3,3/1}
          {1/0,1/1,1/2,1/3,0/1,2/1,3/1,3/0}$$
follows the Fishburn distribution.
\end{proposition}

Unfortunately it is not obvious that Theorem
\ref{theorem-q-factorial-construction} can be applied here so we adopt
a more direct approach.

Recall $\meshpata$ defined on page \pageref{meshpata}.  An occurrence
$abc$ of $\meshpata$ in a permutation satisfies one of two conditions:
\begin{enumerate}
\item There exists $d$ with $d < c$ occurring to the right of $c$ in
  the permutation.
\item There is no such $d$.
\end{enumerate}

Thus $\meshpata$ can be viewed as the following linear combination of
mesh patterns.
$$
\fmt + \fmo =
  \pattern {}{4}{1/3,2/4,3/2,4/1}
           {1/0,1/1,1/2,1/3,1/4,0/2,2/2,3/2,4/2,4/0,4/1}
  +
  \pattern{}{3}{1/2,2/3,3/1}
          {1/0,1/1,1/2,1/3,0/1,2/1,3/1,3/0}.
$$

In addition to showing that $\meshpata$ follows the Fishburn
distribution, Eriksen and Sj\"{o}strand show that occurrences of the
following are equidistributed.

$$\meshpatc = \pattern{}{3}{1/2,2/3,3/1}
{2/0,2/1,2/2,2/3,0/1,1/1,3/1}. $$

In a similar manner as before consider the decomposition of an
occurrence of $\meshpatc$ in a permutation.
$$
\mft + \mfo =
  \pattern {}{4}{1/3,2/4,3/2,4/1}
           {2/0,2/1,2/2,2/3,2/4,0/2,1/2,3/2,4/2,4/0,4/1}
  +
  \pattern{}{3}{1/2,2/3,3/1}
          {2/0,2/1,2/2,2/3,0/1,1/1,3/1,3/0}.
$$

The patterns in Proposition \ref{prop-linear-comb-mesh} are the
combination of patterns $\mft$ and $\fmo$.  We prove Proposition
\ref{prop-linear-comb-mesh} via an involution on permutations which
takes occurrences of $\fmt$ to occurrences of $\mft$ and vice versa
whilst preserving the number of occurrences of $\fmo$.  The proof is
provided later in this section. We begin with an observation on
occurrences of $\fmt$ and $\mft$.

\begin{lemma}\label{lem-linear-comb-mesh-sec-entry}
  For some fixed permutation let $abcd$ and $a'b'c'd'$ be occurrences
  of $\fmt$. If $b=b'$ then the occurrences are equal i.e.\ $a=a'$,
  $b=b'$, $c=c'$ and $d=d'$.

  Similarly let $efgh$ and $e'f'g'h'$ to be occurrences of $\mft$. If
  $f=f'$ then the occurrences are equal.
\end{lemma}
\begin{proof}
  In an occurrence of $\fmt$ the entry corresponding to $b$ must
  immediately follow entry corresponding to $a$ in the permutation, as
  $b=b'$ it then follows that $a=a'$. The value of $a$ fixes the value
  of $c$ and thus $c=c'$. The entry for $d$ is fixed as the first
  right-to-left minima occurring after $c$ in the permutation, thus
  $d=d'$.

  The proof to the second statement is similar to the above, mutatis
  mutandis.
\end{proof}

As the previous lemma shows that the second entry in occurrences of
both $\fmt$ and $\mft$ fix the remaining entries we define an
involution on basis of the following cases.

\begin{enumerate}
\item Occurrences of $\fmt$ in which the second entry is also the
  second entry of an occurrence of $\mft$ are left unmodified.
\item For all occurrences $abcd$ of $\fmt$ in which $b$ is not the
  second entry in an occurrence of $\mft$ move the entry in the
  permutation corresponding to $b$ to the position immediately before
  the entry corresponding to $c$.
\item For all occurrences $efgh$ of $\mft$ in which $f$ is not the
  second entry in an occurrence of $\fmt$ do the opposite of the
  previous case; move the entry corresponding to $f$ to the position
  immediately to the right of the entry corresponding to $e$ in the
  permutation.
\end{enumerate}

To demonstrate that this is an involution we are required to show
that it is well defined in preserving occurrences of patterns.

\begin{lemma}\label{lem-preserve-fmo}
  The above involution preserves the number of occurrences of $\fmo$. 
\end{lemma}
\begin{proof}
  For a fixed permutation let $abcd$ be an occurrence of $\fmt$ and
  $efgh$ an occurrence of $\mft$. Take $ijk$ to be some occurrence of
  $\fmo$.

  It follows immediately by definition of the decomposition of
  $\meshpata$ that a $b$ in the occurrence of $\fmt$ cannot be equal
  to $j$.  As two elements occur below and to the left it cannot be
  equal to $k$, which is a right-to-left minima, nor $i$ which is one
  greater to than $k$. Thus the element to be moved in an occurrence
  of $\fmt$ in the involution is not involved as part of an occurrence
  of $\fmo$. 

  It remains to check if its new location after applying the
  involution breaks an occurrence of $\fmo$. Assume $c=j$, then after
  applying the involution $b$ is moved to immediately before the $c$
  then the occurrence of $\fmo$ is broken but as $b>c$ a new
  occurrence is created and thus the total number is preserved.

  The entry corresponding to $f$ in the occurrence of $\mft$ may be
  equal to $j$, however after applying the involution the $g$ in the
  occurrence of $\mft$ plays the same role as it is larger than the
  next right-to-left minima. As $f$ is immediately positioned before
  an element smaller than it in the permutation it cannot be equal to
  $i$.  Furthermore $f$ cannot be equal to $k$ as there are entries
  smaller and to the right of it. Thus the element to be moved in an
  occurrence of $\fmt$ in the involution is either not involved as
  part of an occurrence of $\fmo$ or a new occurrence is created after
  the involution is applied. 

  Again we ask if the new placement of $f$
  after the involution is applied breaks any pre-existing occurrence
  of $\fmo$. Assume $g=j$, then moving $f$ immediately to the left of
  $g$ in the permutation breaks the occurrence of $\fmo$ but as $f>g$
  a new occurrence is created and thus the total number is preserved

  Therefore the involution preserves the number of occurrences of
  $\fmo$.
\end{proof}

\begin{lemma}\label{lem-map-fmt-mft}
For a fixed permutation the involution allows us to map occurrences of
$\fmt$ to occurrences of $\mft$ and vice versa.
\end{lemma}
\begin{proof}

  Consider the different cases under the involution. 

  An occurrence of $\fmt$ in which the second entry is also the second
  entry of an occurrence of $\mft$ are mapped to one another.

  For $abcd$ a fixed occurrence of $\fmt$ and $efgh$ some occurrence
  of $\mft$ such that $b \neq f$ we have that as the position
  immediately before $b$ in the permutation is occupied by $a$ with $a
  <b$ therefore $b \neq g$. As $b$ has two smaller entries to its
  right it is not $h$, which is a right-to-left minima. Assume $b=e$,
  applying the involution breaks this occurrence of $\mft$, however a
  new occurrence is formed.

  For $efgh$ a fixed occurrence of $\mft$ and $abcd$ some occurrence
  of $\fmt$ such that $f \neq b$ we have that as the position
  immediately after $f$ in the permutation is occupied by $g$ with $g
  <f$ therefore $f \neq a$.  As $f$ has two smaller entries to its
  right it is not a right-to-left minima and thus cannot be $d$ in an
  occurrence of $\mft$. Assume $f=c$ applying the involution breaks
  this occurrence of $\fmt$, however a new occurrence is formed.
\end{proof}

The above Lemmas allow us to prove Proposition
\ref{prop-linear-comb-mesh}.

\begin{proof}[Proposition \ref{prop-linear-comb-mesh}]
  Occurrences of $\meshpata = \fmt + \fmo$ in permutations are known
  to be enumerated by the Fishburn distribution. Lemma
  \ref{lem-map-fmt-mft} shows that for a given permutation the
  involution maps $\fmt \to \mft$ and vice versa whilst Lemma
  \ref{lem-preserve-fmo} gives that this preserves $\fmo$. 

  Thus the number of occurrences of $\mft + \fmo$ follow the Fishburn
  distribution.
\end{proof}

\begin{remark}
  It is undeniable that the proof presented above is an unelegant case
  analysis.  Ideally we would want a general approach to construct a
  set of linear combinations of patterns following the Fishburn
  distribution from any given Mahonian linear combination of patterns.
  However, as noted earlier, it is not evident that the technique
  detailed earlier in this chapter can be used here.

  We highlight this as an area worthy of additional study. 
\end{remark}

